Multi-dimensional optical neural network

The development of deep neural networks is witnessing fast growth in network size, which requires novel hardware computing platforms with large bandwidth and low energy consumption. Optical computing has been a potential candidate for next-generation computing systems. Specifically, wavelength-division multiplexing (WDM) has been widely adopted in optical neural network architecture to increase the computation bandwidth. Although existing WDM neural networks architectures have shown promise, they face challenges in the integration of light sources and further increase of the computing bandwidth. To overcome these issues, we introduce a mode-division multiplexing (MDM) strategy, offering a new degree of freedom in optical computing within the micro-ring resonator platform. We propose a MDM approach for small-scale networks and a multi-dimensional architecture for large-scale applications, supplementing WDM with MDM to enhance channel capacity for computations. In this work, we design and experimentally demonstrate key components for the MDM computing system, i.e., a multimode beam splitter, a thermo-optical tuner for the high-order mode, and a multimode waveguide bend. We further show a 2-by-2 matrix multiplexing system fabricated in a foundry that works for both MDM and MDM-WDM computing, which confirms that our approach successfully increases the input vector size for computing and ensures compatibility with existing WDM networks.

==> extra/cleanmaintex <==
#!/usr/bin/env bash
# Nice Perl thing that removes the custom commands used for the resubmission.
# VERY IMPORTANT: since I'm terrible at Perl regexp, we have to keep these two
# lines SEPARATED and DON'T MERGE the "-pe" commands (I don't know why, but
# matching (iac|mat|tom) doesn't work.

for texfile in InvFWM.tex InvFWM_suppl.tex; do

    perl -i.original -ne 'print unless /^\\newcommand\{\\(zhetao|matteo|bk)\}\[1\]/;' $texfile
    # Loop for nested \iac{ or \mat{; '-0777' causes to process the whole file (and not line-by-line).
    while grep -e '\\zhetao{' -e '\\matteo{' -e '\\bk{' $texfile > /dev/null; do
        perl -0777 -i -pe 's/\\zhetao (\{( (?: [^{}]*+ | (?1) )* )\}) /\2/gx;' -pe 's/\\matteo (\{( (?: [^{}]*+ | (?1) )* )\}) /\2/gx;' -pe 's/\\bk (\{( (?: [^{}]*+ | (?1) )* )\}) /\2/gx;' $texfile
    done

done



# Then, with sed, we remove the remaining stuff. Note that sed adds a newline at the EOF if it doesn't exist.

# Trick to make in-pace sed work both on MacOS and Linux
sedi=(-i)
case "$(uname)" in
  Darwin*) sedi=(-i "")
esac

## Remove the command including the supplementary file after the bibliography and \warn
#sed "${sedi[@]}" -e '/^\\bibliography/,/^\\includesupplementary/{/^\\bibliography/!{/^\n/!d;};}' InvFWM.tex

# Remove everything from %__deleteBEGIN to %__deleteEND
for texfile in InvFWM.tex InvFWM_suppl.tex; do
    sed "${sedi[@]}" -e '/^\%__deleteBEGIN/,/^\%__deleteEND/d;' $texfile
done


==> extra/makedist <==
#!/usr/bin/env bash


# Trick to make in-pace sed work both on MacOS and Linux
sedi=(-i)
case "$(uname)" in
  Darwin*) sedi=(-i "")
esac



# Purge source files
bash extra/cleanmaintex

# Replace \date{\today} with \date{...} for arXiv
today=$(LANG=en_US date +'%B %d, %Y')
for texfile in InvFWM.tex InvFWM_suppl.tex; do
    sed "${sedi[@]}" -e 's/\\date{\\today}/\\date{'"$today"'}/g' $texfile
done

# First, compile the Supplementary Material
latexmk -pdf InvFWM_suppl.tex

# Then, let the Makefile compile the rest
make

# Now collect the annotations in the Supplementary Material
# You might need to do pdfannotextractor --install the first
# time you use the program
pdfannotextractor InvFWM_suppl.pdf

# Create the intermediate distribution package
make dist

# Tweak the distribution package so that the
# supplemental material binary files are in extra
mkdir tmp
cd tmp
cp ../InvFWM.tar.gz .
tar -zxvf InvFWM.tar.gz
mv InvFWM_suppl.pdf extra/
mv InvFWM_suppl.pax extra/

# Correct the position of supplementary png figures
mv FigS*.png figures

# Since we've changed the location of the files, we have to
# adjust the sources as well
sed "${sedi[@]}" -e 's/\\def\\supplementfilename{InvFWM_suppl}/\\def\\supplementfilename{extra\/InvFWM_suppl}/g' InvFWM.tex

# Repack again
COPYFILE_DISABLE=1 tar cfv - --exclude InvFWM.tar.gz * | gzip -9 -n >InvFWM.tar.gz
mv InvFWM.tar.gz ..

# Do variant for journal
sed "${sedi[@]}" -e 's/\\input{extra\/includesupplementary}/\%\\input{extra\/includesupplementary}/g' InvFWM.tex
sed "${sedi[@]}" -e 's/\\includesupplementary/\%\\includesupplementary/g' InvFWM.tex
mv extra/InvFWM_suppl.pdf .
rm -R extra
rm InvFWM_suppl.tex rm InvFWM_suppl.bbl
rm 00README.XXX

# Correct the position of supplementary png figures
mv FigS*.png figures

# Repack again
COPYFILE_DISABLE=1 tar cfv - --exclude InvFWM-APL.tar.gz * | gzip -9 -n >InvFWM-APL.tar.gz
mv InvFWM-APL.tar.gz ..

# Remove temp files
cd ..
rm -R tmp

# Remove unnecessary dist file
rm InvFWM_suppl.tar.gz


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 'bbl', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
